List-$k$-Coloring $H$-free graphs for all $k>4$

Given an integer $k>4$ and a graph $H$, we prove that, assuming P$\neq$NP, the List-$k$-Coloring Problem restricted to $H$-free graphs can be solved in polynomial time if and only if either every component of $H$ is a path on at most three vertices, or removing the isolated vertices of $H$ leaves an induced subgraph of the five-vertex path. In fact, the "if" implication holds for all $k\geq 1$.

==> rP3ref.tex <==
@article {HGL,
	AUTHOR = {Ding, Guoli and Seymour, Paul and Winkler, Peter},
	TITLE = {Bounding the vertex cover number of a hypergraph},
	JOURNAL = {Combinatorica},
	FJOURNAL = {Combinatorica. An International Journal on Combinatorics and
	the Theory of Computing},
	VOLUME = {14},
	YEAR = {1994}, 
	NUMBER = {1},
	PAGES = {23--34},
	ISSN = {0209-9683},
	MRCLASS = {05C65 (05C35 05C70)},
	MRNUMBER = {1273198},
	MRREVIEWER = {Ioan Tomescu},
	DOI = {10.1007/BF01305948},
	URL = {https://doi.org/10.1007/BF01305948},
}
@article {frugal,
	AUTHOR = {Hind, Hugh and Molloy, Michael and Reed, Bruce},
	TITLE = {Colouring a graph frugally},
	JOURNAL = {Combinatorica},
	FJOURNAL = {Combinatorica. An International Journal on Combinatorics and
	the Theory of Computing},
	VOLUME = {17},
	YEAR = {1997},
	NUMBER = {4},
	PAGES = {469--482},
	ISSN = {0209-9683},
	MRCLASS = {05C15},
	MRNUMBER = {1645682},
	MRREVIEWER = {David E. Woolbright},
	DOI = {10.1007/BF01195001},
	URL = {https://doi.org/10.1007/BF01195001},
}
@article {listfrugal,
	AUTHOR = {Cohen, Nathann and Havet, Fr\'{e}d\'{e}ric},
	TITLE = {Linear and 2-frugal choosability of graphs of small maximum
	average degree},
	JOURNAL = {Graphs Combin.},
	FJOURNAL = {Graphs and Combinatorics},
	VOLUME = {27},
	YEAR = {2011},
	NUMBER = {6},
	PAGES = {831--849},
	ISSN = {0911-0119},
	MRCLASS = {05C15},
	MRNUMBER = {2844795},
	MRREVIEWER = {Anna O. Ivanova},
	DOI = {10.1007/s00373-010-1009-7},
	URL = {https://doi.org/10.1007/s00373-010-1009-7},
}
@article{golovachsurvey,
	title={A survey on the computational complexity of coloring graphs with forbidden subgraphs},
	author={Golovach, Petr A and Johnson, Matthew and Paulusma, Dani{\"e}l and Song, Jian},
	journal={Journal of Graph Theory},
	volume={84},
	number={4},
	pages={331--363},
	year={2017},
	publisher={Wiley Online Library}
}

@incollection{ karp,
	title={Reducibility among combinatorial problems},
	author={Karp, Richard M},
	booktitle={Complexity of computer computations},
	pages={85--103},
	year={1972},
	publisher={Springer}
}

@article{ClawFree,
	title={The {{NP}}-Completeness of Edge-Coloring},
	author={Ian Holyer},
	journal={SIAM J. Comput.},
	year={1981},
	volume={10},
	pages={718-720}
}

@article{CycleFree,
	title={Coloring edges and vertices of graphs without short or long cycles},
	author={  Kami\'{n}ski, Marcin and Lozin, Vadim},
	journal={Contributions Discret. Math.},
	year={2007},
	volume={2}
}

@inproceedings{H,
	title={Complexity of coloring graphs without forbidden induced subgraphs},
	author={Kr\'{a}l, Daniel and Kratochv{\'\i}l, Jan and Tuza, Zsolt and Woeginger, Gerhard J and others},
	booktitle={International Workshop on Graph-Theoretic Concepts in Computer Science},
	pages={254--262},
	year={2001},
	organization={Springer}
}

@article{ListH,
	author = {Golovach, Petr and Paulusma, Daniël and Song, Jian},
	year = {2014},
	month = {10},
	pages = {},
	title = {Closing Complexity Gaps for Coloring Problems on {$H$}-Free Graphs},
	volume = {237},
	isbn = {978-3-642-35260-7},
	journal = {Information and Computation},
	doi = {10.1016/j.ic.2014.02.004}
}

@article{kP5,
	title={Deciding k-colorability of {$P_5$}-free graphs in polynomial time},
	author={Ho{\`a}ng, Ch{\'\i}nh T and Kami{\'n}ski, Marcin and Lozin, Vadim and Sawada, Joe and Shu, Xiao},
	journal={Algorithmica},
	volume={57},
	number={1},
	pages={74--81},
	year={2010},
	publisher={Springer}
}

@inproceedings{4P6,
	title={Four-coloring {$P_6$}-free graphs},
	author={Chudnovsky, Maria and Spirkl, Sophie and Zhong, Mingxian},
	booktitle={Proceedings of the Thirtieth Annual ACM-SIAM Symposium on Discrete Algorithms},
	pages={1239--1256},
	year={2019},
	organization={SIAM}
}

@article{3P7,
	title={Three-coloring and list three-coloring of graphs without induced paths on seven vertices},
	author={Bonomo, Flavia and Chudnovsky, Maria and Maceli, Peter and Schaudt, Oliver and Stein, Maya and Zhong, Mingxian},
	journal={Combinatorica},
	volume={38},
	number={4},
	pages={779--801},
	year={2018},
	publisher={Springer}
}

@article{LkP5+rP1&L5P4+P2-NP,
	volume = {71},
	number = {1},
	month = {January},
	author = {Couturier, Jean-François and Golovach, Petr and Kratsch, Dieter and Paulusma, Daniël},
	title = {List coloring in the absence of a linear forest},
	publisher = {Springer},
	year = {2015},
	journal = {Algorithmica},
	pages = {21-35},
}

@article{krP2,
	author = {Alekseev, Vladimir},
	year = {2007},
	month = {01},
	pages = {355-359},
	title = {An upper bound for the number of maximal independent sets in a graph},
	volume = {17},
	journal = {Discrete Mathematics and Applications},
	doi = {10.1515/dma.2007.030}
}

@article{3*P2+P4&3*rP3,
	author = {Broersma, Hajo and Golovach, Petr A. and Paulusma, Dani\"{e}l and Song, Jian},
	title = {Updating the Complexity Status of Coloring Graphs without a Fixed Induced Linear Forest},
	year = {2012},
	issue_date = {January, 2012},
	publisher = {Elsevier Science Publishers Ltd.},
	address = {GBR},
	volume = {414},
	number = {1},
	issn = {0304-3975},
	url = {https://doi.org/10.1016/j.tcs.2011.10.005},
	doi = {10.1016/j.tcs.2011.10.005},
	journal = {Theor. Comput. Sci.},
	month = jan,
	pages = {9–19},
	numpages = {11},
}

@article{L4P6-NP,
	author = {Golovach, Petr and Paulusma, Daniël and Song, Jian},
	year = {2014},
	month = {10},
	pages = {},
	title = {Closing Complexity Gaps for Coloring Problems on {$H$}-Free Graphs},
	volume = {237},
	isbn = {978-3-642-35260-7},
	journal = {Information and Computation},
}

@article{ 5P6&4P7-NP,
	author = {Huang, Shenwei},
	year = {2016},
	month = {01},
	pages = {336-346},
	title = {Improved complexity results on $k$-coloring {$P_t$}-free graphs},
	volume = {51},
	journal = {European Journal of Combinatorics},
	doi = {10.1016/j.ejc.2015.06.005}
}

@article{L3P6+rP3,
	author = {Chudnovsky, Maria and Huang, Shenwei and Spirkl, Sophie and Zhong, Mingxian},
	year = {2021},
	month = {01},
	pages = {216-251},
	title = {List 3-Coloring Graphs with No Induced {$P_6+rP_3$}},
	volume = {83},
	journal = {Algorithmica},
	doi = {10.1007/s00453-020-00754-y}
}

@book{NAE-NP,
	author = {Garey, Michael and Johnson, David},
	year = {1979},
	month = {01},
	pages = {},
	title = {Computer and Intractability: A Guide to the Theory of NP-Completeness}
}

@article {2sat1,
	AUTHOR = {Edwards, Keith},
	TITLE = {The complexity of colouring problems on dense graphs},
	JOURNAL = {Theoret. Comput. Sci.},
	FJOURNAL = {Theoretical Computer Science},
	VOLUME = {43},
	YEAR = {1986},
	NUMBER = {2-3},
	PAGES = {337--343},
	ISSN = {0304-3975},
	MRCLASS = {05C15 (68Q25 68R10)},
	MRNUMBER = {855980},
	MRREVIEWER = {Narsingh Deo},
	DOI = {10.1016/0304-3975(86)90184-2},
	URL = {https://doi.org/10.1016/0304-3975(86)90184-2},
}

@inproceedings {2sat2,
	AUTHOR = {Erd\H{o}s, Paul and Rubin, Arthur L. and Taylor, Herbert},
	TITLE = {Choosability in graphs},
	BOOKTITLE = {Proceedings of the {W}est {C}oast {C}onference on
	{C}ombinatorics, {G}raph {T}heory and {C}omputing ({H}umboldt
	{S}tate {U}niv., {A}rcata, {C}alif., 1979)},
	SERIES = {Congress. Numer., XXVI},
	PAGES = {125--157},
	PUBLISHER = {Utilitas Math., Winnipeg, Man.},
	YEAR = {1980},
	MRCLASS = {05C15},
	MRNUMBER = {593902},
	MRREVIEWER = {R. C. Entringer},
}

@article {2sat3,
	AUTHOR = {Vizing, V. G.},
	TITLE = {Coloring the vertices of a graph in prescribed colors},
	JOURNAL = {Diskret. Analiz},
	FJOURNAL = {Akademiya Nauk SSSR. Sibirskoe Otdelenie. Institut Matematiki.
	Diskretny\u{\i} Analiz. Sbornik Trudov},
	YEAR = {1976},
	NUMBER = {29, Metody Diskret. Anal. v Teorii Kodov i Shem},
	PAGES = {3--10, 101},
	MRCLASS = {05C15},
	MRNUMBER = {498216},
	MRREVIEWER = {D. Cvetkovi\'{c}},
}


@article {L5CrP3,
    AUTHOR = {Hajebi, Sepehr and Li, Yanjia and Spirkl, Sophie},
     TITLE = {Complexity dichotomy for list-5-coloring with a forbidden
              induced subgraph},
   JOURNAL = {SIAM J. Discrete Math.},
  FJOURNAL = {SIAM Journal on Discrete Mathematics},
    VOLUME = {36},
      YEAR = {2022},
    NUMBER = {3},
     PAGES = {2004--2027},
      ISSN = {0895-4801,1095-7146},
   MRCLASS = {68R10 (05C15)},
  MRNUMBER = {4474376},
MRREVIEWER = {Ewan\ Davies},
       DOI = {10.1137/21M1443352},
       URL = {https://doi.org/10.1137/21M1443352},
}

@article {H&K,
    AUTHOR = {Hopcroft, John E. and Karp, Richard M.},
     TITLE = {An {$n\sp{5/2}$} algorithm for maximum matchings in bipartite
              graphs},
   JOURNAL = {SIAM J. Comput.},
  FJOURNAL = {SIAM Journal on Computing},
    VOLUME = {2},
      YEAR = {1973},
     PAGES = {225--231},
      ISSN = {0097-5397},
   MRCLASS = {05C99},
  MRNUMBER = {337699},
MRREVIEWER = {Torrence\ D.\ Parsons},
       DOI = {10.1137/0202019},
       URL = {https://doi.org/10.1137/0202019},
}
